One Ranking, Any Budget: Matryoshka Evidence-to-Context Frame Selection for Long-Video Understanding

Frame selection is essential for applying Large Multimodal Models (LMMs) to long videos due to severe frame redundancy and limited context windows. Since the appropriate frame budget varies with the downstream LMM, reasoning demands, and latency constraints, a practical selector should serve multiple budgets. However, existing methods typically optimize an isolated frame subset for each predefined budget: when the budget changes, previously selected evidence may be replaced rather than progressively augmented. A fixed-weight ranking allows prefix reuse across budgets but applies the same weighting at every position, overlooking the distinct roles of early and later ranks. We formulate long-video frame selection as a Matryoshka ranking problem: constructing a single priority sequence whose small prefixes concentrate query-conditioned evidence, while progressively larger prefixes preserve this evidence and add broader temporal context. Efficiently constructing such a ranking is itself challenging, as densely sampling long videos and evaluating frame-query relevance incurs substantial overhead. We therefore introduce Matryoshka Evidence-to-Context (MEC) Frame Selection, a training-free framework that builds a reusable sparse video index, discovers candidates through sparse probing and local zooming, and greedily constructs a position-adaptive ranking - early positions emphasize evidence; later positions progressively favor temporal coverage while preserving visual diversity. A single ranking can thus be truncated to any target budget without rerunning the selector. Across four benchmarks and six frame budgets, MEC improves average accuracy over uniform sampling by 3.77 points, matches strong state-of-the-art selectors, and reduces end-to-end selection latency by 47.37-51.19%.

==> template/mac_automl_core.tex <==
% =============================================================================
% MAC-AutoML core template
% Public responsibility:
% 1. Load all shared packages and layout rules.
% 2. Expose shared front-matter and header/footer configuration APIs.
% 3. Keep all theme-independent visual logic in one place.
%
% Theme wrappers are expected to define:
% - \macframecolordef
% - \macaccentcolordef
% - \macaccenttext
% =============================================================================

\@ifundefined{macframecolordef}{\ClassError{\@classname}{Missing theme hook \string\macframecolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccentcolordef}{\ClassError{\@classname}{Missing theme hook \string\macaccentcolordef}{Define it in the theme .cls before loading mac_automl_core.tex}}{}
\@ifundefined{macaccenttext}{\ClassError{\@classname}{Missing theme hook \string\macaccenttext}{Define it in the theme .cls before loading mac_automl_core.tex}}{}

\newif\ifmacsubmissionmode
\newif\ifmacanonymousmode
\macsubmissionmodefalse
\macanonymousmodefalse

\DeclareOption{submission}{\macsubmissionmodetrue}
\DeclareOption{review}{\macsubmissionmodetrue}
\DeclareOption{cameraready}{\macsubmissionmodefalse}
\DeclareOption{camera-ready}{\macsubmissionmodefalse}
\DeclareOption{final}{\macsubmissionmodefalse}
\DeclareOption{anonymous}{\macanonymousmodetrue}
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions\relax

\LoadClass{article}
\RequirePackage{iftex}
\ifdefined\pdfoutput
\pdfoutput=1
\fi

% =============================================================================
% Core packages and layout
% =============================================================================

\RequirePackage[top=2.12cm, bottom=3.20cm, left=2.5cm, right=2.5cm, columnsep=0.65cm]{geometry}
\ifXeTeX\else
\RequirePackage{microtype}
\fi
\RequirePackage{placeins}
\RequirePackage{setspace}
\RequirePackage{parskip}
\RequirePackage[english]{babel}
\RequirePackage{lipsum}
\RequirePackage{etoolbox}
\RequirePackage{enumitem}
\newcommand{\nohyphens}{\hyphenpenalty=10000\exhyphenpenalty=10000\relax}

\RequirePackage{fancyhdr}
\@ifundefined{DisableLigatures}{}{\DisableLigatures[f]{family=sf*}}

% =============================================================================
% Graphics
% =============================================================================

\RequirePackage{graphicx}
\RequirePackage[export]{adjustbox}
\RequirePackage{subcaption}

% =============================================================================
% Tables
% =============================================================================

\RequirePackage{booktabs}
\RequirePackage{nicematrix}
\RequirePackage{multirow}
\RequirePackage{makecell}
\RequirePackage{colortbl}
\RequirePackage{bm}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\ifmacsubmissionmode
  \RequirePackage[switch,mathlines]{lineno}
  \AtBeginDocument{%
    \modulolinenumbers[1]%
    \linenumbers
  }
\fi
\RequirePackage{pifont}
\RequirePackage{marvosym}
\newcommand{\nm}[1]{#1}

% =============================================================================
% Theme colors
% =============================================================================

\RequirePackage[most]{tcolorbox}
\RequirePackage{xcolor}
\macframecolordef
\macaccentcolordef
\newcommand{\omniaccent}[1]{\macaccenttext{#1}}
\definecolor{black}{rgb}{0,0,0}
\newcommand{\black}[1]{{\bfseries\color[HTML]{000000} #1}}
\definecolor{macreviewnote}{RGB}{172,73,0}

% =============================================================================
% References
% =============================================================================

\RequirePackage{hyperref}
\RequirePackage{xurl}
\RequirePackage[noabbrev,nameinlink]{cleveref}
\hypersetup{
  colorlinks,
  linkcolor=omniaccent,
  citecolor=omniaccent,
  urlcolor=omniaccent
}

\RequirePackage[numbers, sort&compress]{natbib}
\def\bibfont{\small}
\special{pdf:minorversion 7}
\emergencystretch=1.5em
\hbadness=2000

% =============================================================================
% Bibliography
% =============================================================================
\addto{\captionsenglish}{\renewcommand{\refname}{References}}
\newcommand{\citeas}[1]{\Needspace*{8\baselineskip}\noindent\bibentry{#1}}

% =============================================================================
% Section and caption style
% =============================================================================

\newcommand{\sectionfont}
{\fontsize{13}{14}\selectfont}

\newcommand{\subsectionfont}
{\fontsize{11}{13}\selectfont}

\RequirePackage{titlesec}
\titleformat*{\paragraph}{\itshape}
\titleformat*{\section}{\sectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsection}{\subsectionfont\sffamily\bfseries\omniaccent}
\titleformat*{\subsubsection}{\normalsize\sffamily\bfseries\omniaccent}
\titlespacing*{\section}{0pt}{3ex plus4pt minus3pt}{5pt}
\titlespacing*{\subsection}{0pt}{2.5ex plus3pt minus2pt}{2pt}
\titlespacing*{\subsubsection}{0pt}{2ex plus2.5pt minus1.5pt}{2pt}

\RequirePackage{caption}
\DeclareCaptionLabelSeparator{period}{. }
\captionsetup{
  labelfont={bf,sf},
  labelsep=period,
  figurename=Figure,
  tablename=Table,
  format=plain,
  singlelinecheck=off,
  justification=raggedright,
  font=small
}
\captionsetup[figure]{
  skip=6pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}
\captionsetup[table]{
  skip=4pt,
  format=plain,
  singlelinecheck=off,
  justification=raggedright
}

\ifXeTeX
  \RequirePackage{fontspec}
  % Resolve TeX Live font files directly so the template also compiles on
  % systems where these fonts are not registered with the OS font manager.
  \setmainfont[
    UprightFont = texgyretermes-regular.otf,
    BoldFont = texgyretermes-bold.otf,
    ItalicFont = texgyretermes-italic.otf,
    BoldItalicFont = texgyretermes-bolditalic.otf,
    SmallCapsFeatures = {Letters=SmallCaps}
  ]{texgyretermes-regular.otf}
  \setsansfont[
    UprightFont = texgyreheros-regular.otf,
    BoldFont = texgyreheros-bold.otf
  ]{texgyreheros-regular.otf}
  \setmonofont[
    UprightFont = texgyrecursor-regular.otf,
    BoldFont = texgyrecursor-bold.otf
  ]{texgyrecursor-regular.otf}
  \newfontfamily\omnibytesansmedium[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Medium,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Medium}
  \newfontfamily\omnititlefont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniheadingfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniauthorfont[
    Path = assets/fonts/,
    Extension = .ttf,
    UprightFont = ByteSans-Bold,
    BoldFont = ByteSans-Bold
  ]{ByteSans-Bold}
  \newfontfamily\omniaffiliationfont[
    UprightFont = texgyreheros-regular.otf,
    BoldFont = texgyreheros-bold.otf
  ]{texgyreheros-regular.otf}
  \newfontfamily\omniemailfont[
    UprightFont = texgyreheros-regular.otf,
    BoldFont = texgyreheros-bold.otf
  ]{texgyreheros-regular.otf}
  \newfontfamily\omnimonofont[
    UprightFont = texgyrecursor-regular.otf,
    BoldFont = texgyrecursor-bold.otf
  ]{texgyrecursor-regular.otf}
\else
  \RequirePackage[T1]{fontenc}
  \renewcommand{\sfdefault}{lmss}%
  \renewcommand{\rmdefault}{cmr}
\fi

% =============================================================================
% Front-matter data model
% =============================================================================

\renewcommand\addtolist[5][]{
  \begingroup
    \if\relax#3\relax\def\sep{}\else\def\sep{#5}\fi
    \let\protect\@unexpandable@protect
    \xdef#3{\expandafter{#3}\sep #4[#1]{#2}}%
  \endgroup
}

\newcommand{\authorfont}
{\fontsize{12}{14}\selectfont}

\newcommand{\authorgroupfont}
{\fontsize{9.1}{10.8}\selectfont}
\newcommand{\affmark}[1]{\textsuperscript{#1}}

\newcommand\authorlist{}
\ifXeTeX
\newcommand\authorformat[2][]{\authorfont {\color{black!84}\omniauthorfont\bfseries #2\affmark{#1}}}
\else
\newcommand\authorformat[2][]{\authorfont {\color{black!82}\sffamily\mdseries #2\affmark{#1}}}
\fi
\renewcommand\author[2][]{\addtolist[#1]{#2}{\authorlist}{\authorformat}{, }}

\newcommand{\affiliationfont}
{\fontsize{10}{12}\selectfont}

\newcommand\affiliationlist{}
\ifXeTeX
\newcommand\affiliationformat[2][]{{\affiliationfont {\omniaffiliationfont \affmark{#1}#2}}}
\else
\newcommand\affiliationformat[2][]{{\affiliationfont {\sffamily \affmark{#1}#2}}}
\fi
\newcommand\affiliation[2][]{\addtolist[#1]{#2}{\affiliationlist}{\affiliationformat}{, }}

\newcommand{\contributionfont}
{\fontsize{9.6}{12}\selectfont}

\newcommand\contributionlist{}
\newcommand\contributionformat[2][]{{\contributionfont \affmark{#1}#2}}
\newcommand\contribution[2][]{\addtolist[#1]{#2}{\contributionlist}{\contributionformat}{, }}

\newcommand{\emailfont}
{\fontsize{8.2}{10.4}\selectfont}

\newcommand\emaillist{}
\ifXeTeX
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!60}\omniemailfont #1}}}
\else
\newcommand\emails[1]{\def\emaillist{{\emailfont\color{black!65}\ttfamily #1}}}
\fi

\newcommand{\checkdatafont}
{\fontsize{7.92}{10}\selectfont}

\newcommand\checkdatalist{}
\newcommand\checkdataformat[2][]{{\small {\checkdatafont\sffamily \bfseries #1:} #2}}
\newcommand\checkdata[2][]{\addtolist[#1]{#2}{\checkdatalist}{\checkdataformat}{\par}}

\newcommand{\abstractinfont}
{\fontsize{10}{12}\selectfont}

\renewcommand{\abstract}[1]{\def\abstractlist{{\abstractinfont #1}}}
\newcommand{\email}[1]{\href{mailto:#1}{\texttt{#1}}}
\newcommand{\corremailmark}{\Letter}
\newcommand{\authormark}[1]{\textsuperscript{#1}}
\newcommand{\authorentry}[2]{\mbox{#1\authormark{#2}}}
\newcommand{\authorsep}{\hspace{0.78em}}
\newcommand{\authorrow}[1]{\makebox[\linewidth][c]{#1}\par\vspace{2.2pt}}
\newcommand{\affiliationline}[1]{#1\par}
\newcommand{\contactline}[1]{#1\par}

\newcommand{\macauthorrows}{}
\newcommand{\macaffiliationrows}{}
\newcommand{\maccontactrows}{}

% Public front-matter configuration API.
\newcommand{\setauthorrows}[1]{\gdef\macauthorrows{#1}}
\newcommand{\setaffiliationrows}[1]{\gdef\macaffiliationrows{#1}}
\newcommand{\setcontactrows}[1]{\gdef\maccontactrows{#1}}
\newcommand{\usecustomauthorlayout}{
  \def\authorlist{%
    {\fontsize{9.6}{11.6}\selectfont\color{black!96}%
    \ifXeTeX\omniauthorfont\bfseries\else\sffamily\bfseries\fi
    \parbox{\linewidth}{\centering \macauthorrows}}}
  \def\affiliationlist{%
    {\fontsize{8.7}{10.4}\selectfont\color{black!55}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \parbox{0.96\linewidth}{\centering
    \macaffiliationrows\par
    \vspace{2.2mm}
    {\fontsize{8.9}{10.7}\selectfont\color{black!78}%
    \ifXeTeX\omnibytesansmedium\else\sffamily\fi
    \maccontactrows}}}}
  \def\emaillist{{}}}
\newcommand{\setfrontauthors}[1]{\setauthorrows{#1}}
\newcommand{\setfrontaffiliations}[1]{\setaffiliationrows{#1}}
\newcommand{\setfrontcontact}[1]{\setcontactrows{#1}}

\ifmacanonymousmode
  \AtBeginDocument{%
    \gdef\authorlist{%
      {\fontsize{12}{14}\selectfont\color{black!96}%
      \ifXeTeX\omniauthorfont\bfseries\else\sffamily\bfseries\fi
      Anonymous Authors}}%
    \gdef\affiliationlist{%
      {\fontsize{9.9}{11.9}\selectfont\color{black!70}%
      \ifXeTeX\omnibytesansmedium\else\sffamily\fi
      Affiliations withheld for double-blind review}}%
    \gdef\emaillist{}%
    \gdef\maccontactrows{}%
    \gdef\checkdatalist{}%
  }
\fi

\renewcommand\date[1]{\checkdata[Date]{#1}}
\newcommand\correspondence[1]{\checkdata[Correspondence]{#1}}

\newcommand{\titlefont}
{\fontsize{17}{20}\selectfont}

\ifXeTeX
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.945\linewidth}{\centering\titlefont{\omnititlefont\bfseries #1}}}}
\else
\renewcommand{\title}[1]{\newcommand{\titlelist}{\parbox{0.92\linewidth}{\centering\titlefont{\sffamily\bfseries #1}}}}
\fi

\newcommand{\abstractfont}
{\fontsize{12}{12}\selectfont}

\ifXeTeX
\newcommand{\beginabstract}{\abstractfont{\omniauthorfont\bfseries\color{omniaccent!88!black}Abstract}}
\else
\newcommand{\beginabstract}{\abstractfont{\sffamily\bfseries\color{omniaccent}\MakeUppercase{Abstract}}}
\fi

\newcommand{\beginappendix}{\appendix{\titlefont\sffamily \omniaccent{Appendix}\par}}
\colorlet{abstractboxfill}{white}

% =============================================================================
% Reusable document-level utilities
% =============================================================================

\newcommand{\macparagraph}[1]{\par\vspace{2pt}\noindent\textbf{#1}\hspace{1.8ex}}
\newcommand{\reviewnote}[1]{%
  \ifmacsubmissionmode
    {\color{macreviewnote}\bfseries [Review note: }{\color{macreviewnote}#1}{\color{macreviewnote}\bfseries ]}%
  \fi
}
\definecolor{macgreen}{RGB}{34,139,34}
\definecolor{macred}{RGB}{220,20,60}
\definecolor{macorange}{RGB}{255,140,0}
\newcommand{\cmark}{\textcolor{macgreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{macred}{\ding{55}}}
\newcommand{\pmark}{\textcolor{macorange}{\raisebox{0.12ex}{\footnotesize\textasciitilde}}}
\newcommand{\fb}{\makebox[0.5em][c]{\textbullet}}
\newcommand{\eb}{\makebox[0.5em][c]{\textopenbullet}}
\newcommand{\eg}{e.g.,\ }
\newcommand{\ie}{i.e.,\ }

\tcbuselibrary{skins}
\tcbset{
  aibox/.style={
    width=\linewidth,
    top=7pt,
    bottom=2pt,
    colback=blue!4!white,
    colframe=black,
    colbacktitle=black,
    enhanced,
    center,
    attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    boxed title style={boxrule=0pt,colframe=white,},
  }
}
\newtcolorbox{AIbox}[2][]{aibox,title=#2,#1}

% =============================================================================
% Template-level branding configuration
% =============================================================================

\newcommand{\macleftheadercontent}{}
\newcommand{\macrightheadericon}{}
\newcommand{\macrunningheadericon}{}
\newcommand{\macheadertextcontent}{MAC-AutoML}
\newcommand{\macreviewheaderlabel}{Submission / Review Copy}

\newcommand{\setleftheadercontent}[1]{\gdef\macleftheadercontent{#1}}
\newcommand{\setrightheadericon}[1]{\gdef\macrightheadericon{#1}}
\newcommand{\setrunningheadericon}[1]{\gdef\macrunningheadericon{#1}}
\newcommand{\setheadergroupname}[1]{\gdef\macheadertextcontent{#1}}
\newcommand{\setreviewheaderlabel}[1]{\gdef\macreviewheaderlabel{#1}}
\newcommand{\headerlogo}[3][0pt]{\raisebox{#1}{\includegraphics[height=#2]{#3}}}
\newcommand{\headerlogospace}[1]{\hspace*{#1}}

% Public header/footer configuration API.
\newcommand{\firstpageheaderlogos}{%
  \makebox[\textwidth][s]{%
    \macleftheadercontent\hfill\macrightheadericon
  }%
}
\ifXeTeX
\newcommand{\omniheadertext}{{\omniauthorfont\fontsize{8.1}{10}\selectfont\color{black!58}\addfontfeatures{LetterSpace=4}\macheadertextcontent\ifmacsubmissionmode\space/\space\macreviewheaderlabel\fi}}
\else
\newcommand{\omniheadertext}{\sffamily\fontsize{8.1}{10}\selectfont\color{black!60} \macheadertextcontent\ifmacsubmissionmode\space/\space\macreviewheaderlabel\fi}
\fi
\fancypagestyle{firststyle}{
    \fancyhead[L]{
        \vskip 0.8mm
        \firstpageheaderlogos
    }
    \fancyhead[R]{}
}
\pagestyle{fancy}
\fancyhf{}
\fancyhead[L]{
  \vskip 2.5mm
  \macrunningheadericon
}
\fancyhead[R]{
  \vskip 4.2mm
  \omniheadertext
}
\fancyfoot[C]{\sffamily\fontsize{8.6}{10}\selectfont\thepage}

\renewcommand{\headrulewidth}{0pt}
\renewcommand{\footrulewidth}{0pt}
\setlength{\headheight}{64pt}
\setlength{\headsep}{6pt}
\setlength{\footskip}{18pt}

% =============================================================================
% Title and abstract box implementation
% =============================================================================
\newcommand{\@toptitlebar}{
  {\color{omniaccent!88!black}\hrule height 2.4pt}
  \vskip 6mm
}
\newcommand{\@bottomtitlebar}{
  \vskip 6mm
  {\color{omniaccent!88!black}\hrule height 2.4pt}
}

% Titlebox %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mymaketitle}{%
  \tcbset{enhanced}
  \tcbset{left=8mm}
  \tcbset{right=8mm}
  \tcbset{top=4.0mm}
  \tcbset{bottom=3.8mm}
  \tcbset{colback=white}
  \tcbset{colframe=omniframe}
  \tcbset{boxrule=3pt}
  \tcbset{before skip=0pt}
  \tcbset{grow to left by=1.5pt}
  \tcbset{grow to right by=1.5pt}
  \tcbset{arc=2.2mm}
      {
      \setlength{\parskip}{0mm}
      \hfuzz=20pt
      \hbadness=10000
      \centering
      \nohyphens

      {
      \vspace*{-4.8mm}
      \@toptitlebar

        \ifmacsubmissionmode
          {\sffamily\fontsize{9.2}{11}\selectfont\bfseries\color{omniaccent!72!black}\macreviewheaderlabel\par}
          \vskip 2.4mm
        \fi
        \titlelist\par
         \@bottomtitlebar
      }
      \vskip 4.0mm
      \authorlist
      \vskip 2.4mm

      \affiliationlist\par
      \ifdefempty{\emaillist}{}{\vskip 3mm \emaillist\par}

      \contributionlist\par
    }
   \vskip 2.6mm

  \begin{tcolorbox}[
    enhanced jigsaw,
    colback=abstractboxfill,
    colframe=omniaccent!99,
    boxrule=1.6pt,
    arc=2.5mm,
    left=8mm,
    right=8mm,
    top=4.1mm,
    bottom=4.2mm,
    interior style={fill=abstractboxfill},
    drop shadow={black!12!white},
    before skip=0pt,
    after skip=0pt
  ]
    \setlength{\parindent}{0cm}
    \setlength{\parskip}{0cm}

    \begin{center}
      \beginabstract
      \vskip 1.8mm
    \end{center}

    \abstractlist\par
    \vskip 0.6mm
    {
      \setlength{\parskip}{0cm}
      \ifdefempty{\checkdatalist}{\vspace*{0.02cm}}{\checkdatalist\par}
      \ifmacsubmissionmode
        {\small {\checkdatafont\sffamily \bfseries Mode:} \macreviewheaderlabel\par}
      \fi
    }
  \end{tcolorbox}
  \tcbset{reset}
  \FloatBarrier

  \thispagestyle{firststyle}
}

\if@twocolumn%
\renewcommand{\maketitle}{
\twocolumn[%
 \vskip 2mm
  \mymaketitle
  \vskip 4mm
]
}%
\else%
\renewcommand{\maketitle}{
  \mymaketitle
  \vskip 4mm
}%
\fi

